Soft Random Sampling: A Theoretical and Empirical Analysis

Soft random sampling (SRS) is a simple yet effective approach for efficient training of large-scale deep neural networks when dealing with massive data. SRS selects a subset uniformly at random with replacement from the full data set in each epoch. In this paper, we conduct a theoretical and empirical analysis of SRS. First, we analyze its sampling dynamics including data coverage and occupancy. Next, we investigate its convergence with non-convex objective functions and give the convergence rate. Finally, we provide its generalization performance. We empirically evaluate SRS for image recognition on CIFAR10 and automatic speech recognition on Librispeech and an in-house payload dataset to demonstrate its effectiveness. Compared to existing coreset-based data selection methods, SRS offers a better accuracy-efficiency trade-off. Especially on real-world industrial scale data sets, it is shown to be a powerful training strategy with significant speedup and competitive performance with almost no additional computing cost.

==> weiz.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htp]
\begin{tabular}{lllll}
                             & { soft sampling} & { ss\_shuffle\_every\_10\_epoch} & { gm\_every\_10epoch} & { gm\_every\_epoch} \\
                             { Full} & { 95.080} & { 95.080}& { 95.080}& { 95.080}\\
{ 5per}  & { 89.590}        & { 87.240}                        & { 87.440}             & { 89.880}           \\
{ 10per} & { 92.110}        & { 90.470}                        & { 90.450}             & { 92.110}           \\
{ 20per} & { 93.270}        & { 92.710}                        & { 92.630}             & { 93.500}           \\
{ 30per} & { 94.290}        & { 93.370}                        & { 93.250}             & { 93.830}          
\end{tabular}
\caption{CIFAR-10 Results w/ 10 epoch warmup}
\label{tab:results-cifar10}
\end{table}
\Cref{tab:results-cifar10} records CIFAR-10 results. The first column is soft sampling with reshuffling every epoch, the second column is soft sampling with reshuffling every 10-th epoch, the third column is gradient matching with core-selection every 10-th epoch, and the forth column is gradient matching with core-selection every epoch.  For all the experiments listed in the table we start training with a model that has been trained with full dataset for 10 epochs.

\begin{table}[htp]
\begin{tabular}{lllll}
                             & { soft sampling} & { ss\_shuffle\_every\_10\_epoch} & { gm\_every\_10epoch} & { gm\_every\_epoch} \\
                              { Full} & { 95.080} & { 95.080}& { 95.080}& { 95.080}\\
{ 5per}  & {72.580}        & { 80.510}                        & { 77.750}             & { 79.710}           \\
{ 10per} & { 91.03}        & { 86.830}                        & { 85.310}             & { 90.340}           \\
{ 20per} & { 93.470}        & { 92.120}                        & { 91.880}             & { 92.910}           \\
{ 30per} & { 93.780}        & { 93.120}                        & { 92.600}             & { 93.550}          
\end{tabular}
\caption{CIFAR-10 Results w/o warmup}
\label{results-cifar10-no-warmup}
\end{table}
\Cref{results-cifar10-no-warmup} records CIFAR-10 results w/o warmup. For all the experiments listed in the table we start training with the same model that has been randomly initialized.

\textbf{Dataset} We compare the soft sampling against gradident matching on the CIFAR-10 dataset (\cite{cifar10}).

\textbf{Model} We use a 18-layer ResNet model(\cite{resnet} of 11 million parameters.

\textbf{Training} We adopt the hyper-parameter setup as prescribed in \cite{loss_landscape_decentralized}. We train with batch size 512, 320 epochs, and a Nesterov Accelerated SGD optimizer with initial learning rate 0.1 and momentum 0.9. Learning rate is annealed by 10x at the 160-th epoch and the 240-th epoch.   

\textbf{Training time} full dataset:6.70sec/epoch. 

